RING#: PR-by-PE Global Localization with Roto-translation Equivariant Gram Learning

Global localization using onboard perception sensors, such as cameras and LiDARs, is crucial in autonomous driving and robotics applications when GPS signals are unreliable. Most approaches achieve global localization by sequential place recognition (PR) and pose estimation (PE). Some methods train separate models for each task, while others employ a single model with dual heads, trained jointly with separate task-specific losses. However, the accuracy of localization heavily depends on the success of place recognition, which often fails in scenarios with significant changes in viewpoint or environmental appearance. Consequently, this renders the final pose estimation of localization ineffective. To address this, we introduce a new paradigm, PR-by-PE localization, which bypasses the need for separate place recognition by directly deriving it from pose estimation. We propose RING#, an end-to-end PR-by-PE localization network that operates in the bird's-eye-view (BEV) space, compatible with both vision and LiDAR sensors. RING# incorporates a novel design that learns two equivariant representations from BEV features, enabling globally convergent and computationally efficient pose estimation. Comprehensive experiments on the NCLT and Oxford datasets show that RING# outperforms state-of-the-art methods in both vision and LiDAR modalities, validating the effectiveness of the proposed approach. The code will be publicly released.

==> figures/case_gl_fail_nclt.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=18cm]{figs/case_gl_fail_nclt.pdf}
    \vspace{-0.1cm}
    \caption{\textbf{Failure localization cases of RING\#-V and RING\#-L on the NCLT dataset.} We display several failure cases of RING\#. On the likelihood plot, the black arrow $\rightarrow$ shows the pose estimated by RING\#, the red arrow {\color{red}{$\rightarrow$}} shows the ground truth pose and the red dot {\color{red}{$\bullet$}} shows the ground truth position. Here we rotate the query neural BEV by $\hat{\theta}$ estimated using RING\# to visualize the neural BEV under a 3-DoF pose transformation.}
    \label{fig:case_gl_fail_nclt}
    \vspace{-0.5cm}
\end{figure*}

==> figures/case_gl_fail_oxford.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=18cm]{figs/case_gl_fail_oxford.pdf}
    \vspace{-0.1cm}
    \caption{\textbf{Failure localization cases of RING\#-V and RING\#-L on the Oxford dataset.} We display several failure cases of RING\#. On the likelihood plot, the black arrow $\rightarrow$ shows the pose estimated by RING\#, the red arrow {\color{red}{$\rightarrow$}} shows the ground truth pose and the red dot {\color{red}{$\bullet$}} shows the ground truth position. Here we rotate the query neural BEV by $\hat{\theta}$ estimated using RING\# to visualize the neural BEV under a 3-DoF pose transformation.}
    \label{fig:case_gl_fail_oxford}
    \vspace{-0.5cm}
\end{figure*}

==> figures/nclt_lidar_gl_traj.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=8.2cm]{figs/nclt_lidar_traj.pdf}
  \vspace{-0.2cm}
  \caption{\textbf{Global localization result of RING\#-L on the NCLT dataset.} The topological nodes are sparse and shown as gray, the ground truth is shown in green, and the prediction is shown in blue.}
  \label{fig:nclt_lidar_gl_traj}
  \vspace{-0.3cm}
\end{figure}

==> figures/nclt_pose_errors.tex <==
\begin{figure*}[htbp]
    \centering
    \subfigure[Vision-based Methods]{
        \includegraphics[width=8.92cm]{figs/nclt/vision/all_2012-01-08_2012-08-20_20.0_5.0_all_2012-01-08_2012-11-16_20.0_5.0_all_2012-08-20_2012-11-16_20.0_5.0/pose_estimation_error_all.pdf}}
    \hspace{-0.25cm}
    \subfigure[LiDAR-based Methods]{
        \includegraphics[width=8.92cm]{figs/nclt/lidar/all_2012-01-08_2012-08-20_20.0_5.0_all_2012-01-08_2012-11-16_20.0_5.0_all_2012-08-20_2012-11-16_20.0_5.0/pose_estimation_error_all.pdf}}
    \vspace{-0.3cm}
    \caption{\textbf{Pose errors at different revisit thresholds of the NCLT dataset.} \blue{SS: SuperPoint + SuperGlue, PN: Patch-NetVLAD, OT: OverlapTransformer.} (a) and (b) present rotation and translation errors of vision-based and LiDAR-based methods at 5m, 10m, and 20m revisit threshold. Compared to other methods, RING\#-V and RING\#-L show minimal changes in pose errors across different revisit thresholds.}
    \label{fig:nclt_PE}
    \vspace{-0.3cm}
\end{figure*}

==> figures/nclt_vision_gl_traj.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=8.2cm]{figs/nclt_vision_traj.pdf}
  \vspace{-0.2cm}
  \caption{\textbf{Global localization result of RING\#-V on the NCLT dataset.} The topological node is shown as \gray{gray} and the ground truth is shown in \green{green}.}
  \label{fig:nclt_vision_gl_traj}
  \vspace{-0.3cm}
\end{figure}

==> figures/oxford_lidar_gl_traj.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=8.2cm]{figs/oxford_lidar_traj.pdf}
  \vspace{-0.2cm}
  \caption{\textbf{Global localization result of RING\#-L on the Oxford dataset.} The topological node is shown as \gray{gray} and the ground truth is shown in \green{green}.}
  \label{fig:oxford_lidar_gl_traj}
  \vspace{-0.3cm}
\end{figure}

==> figures/oxford_pose_errors.tex <==
\begin{figure*}[htbp]
	\centering
    \subfigure[Vision-based Methods]{
		\includegraphics[width=8.92cm]{figs/oxford/vision/all_2019-01-11-14-37-14_2019-01-17-12-48-25_20.0_5.0/pose_estimation_error_all.pdf}}
    \hspace{-0.25cm}    
    \subfigure[LiDAR-based Methods]{
		\includegraphics[width=8.92cm]{figs/oxford/lidar/all_2019-01-11-14-37-14_2019-01-17-12-48-25_20.0_5.0/pose_estimation_error_all.pdf}}
    \vspace{-0.2cm}
	\caption{\textbf{Pose errors at different revisit thresholds of the Oxford dataset.} SS: SuperPoint + SuperGlue, PN: Patch-NetVLAD, OT: OverlapTransformer. (a) and (b) present rotation and translation errors of vision-based and LiDAR-based methods at 5m, 10m, and 20m revisit threshold. Compared to other methods, RING\#-V and RING\#-L show minimal changes in pose errors across different revisit thresholds.}
	\label{fig:oxford_PE}
    \vspace{-0.3cm}
\end{figure*}

==> figures/oxford_vision_gl_traj.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=8.2cm]{figs/oxford_vision_traj.pdf}
  \vspace{-0.2cm}
  \caption{\textbf{Global localization result of RING\#-V on the Oxford dataset.} The topological node is shown as \gray{gray} and the ground truth is shown in \green{green}.}
  \label{fig:oxford_vision_gl_traj}
  \vspace{-0.3cm}
\end{figure}

==> tables/original_runtime.tex <==
\begin{table*}
\renewcommand\arraystretch{1.3}
\centering
\caption{Comparison of Inference Time}
\label{tab:runtime}
\begin{threeparttable}
\begin{tabular}{clcccc}
\toprule[1pt]
\multicolumn{2}{c}{Approach} & Representation [ms] $\downarrow$ & Searching [ms] $\downarrow$ & Pose Estimation [ms] $\downarrow$ & Total [ms] $\downarrow$ \\ \hline
% \multirow{6}{*}{Vision} & NetVLAD-S \cite{arandjelovic2016netvlad} + {SS \cite{detone2018superpoint, sarlin2020superglue}}$^{\dagger}$ & 3.74 & 10.50 & 867.13 & 881.37 \\ % 14780224
\multirow{8}{*}{Vision} & \blue{{Exhaustive SS \cite{detone2018superpoint, sarlin2020superglue}}$^{\dagger}$} & / & / & / & \blue{250000.57} \\ % 14780224
& NetVLAD \cite{arandjelovic2016netvlad} + {SS \cite{detone2018superpoint, sarlin2020superglue}}$^{\dagger}$ & 3.75 & 11.20 & 867.13 & 882.08 \\ % 14780224
& Patch-NetVLAD \cite{hausler2021patch} + {SS \cite{detone2018superpoint, sarlin2020superglue}}$^{\dagger}$ & 4.06 & 11.39 & 867.13 & 882.58 \\ % 14780224
& AnyLoc \cite{keetha2023anyloc} + {SS \cite{detone2018superpoint, sarlin2020superglue}}$^{\dagger}$ & 184.66 & 16.34 & 867.13 & 1068.13 \\
& SFRS \cite{ge2020self} + {SS \cite{detone2018superpoint, sarlin2020superglue}}$^{\dagger}$ & 5.91 & 1.25 & 867.13 & 874.29 \\ % 149002048 
& \blue{BEV-NetVLAD-MLP} & \blue{17.06} & \blue{0.11} & \blue{0.55} & \blue{17.72} \\ % 149002048
& \blue{vDiSCO \cite{xu2023leveraging} + {SS \cite{detone2018superpoint, sarlin2020superglue}}$^{\dagger}$} & \blue{25.39} & \blue{0.22} & \blue{867.13} & \blue{892.74} \\ % 149002048
& \textbf{RING\#-V (Ours)} & 12.64 & 152.92 & 44.22 & 209.78 \\ \hline % 53409998
\multirow{7}{*}{LiDAR} & OverlapTransformer \cite{ma2022overlaptransformer} & 2.31 & 0.16 & / & 2.47 \\
& LCDNet \cite{cattaneo2022lcdnet} & 131.15 & 0.15 & 228.32 & 359.62 \\
& DiSCO \cite{xu2021disco} & 3.01 & 0.53 & 0.55 & 4.09 \\
& RING \cite{lu2022one} & 243.99 & 3.89 & 1.72 & 249.60 \\
& \blue{RING++ \cite{xu2023ring++}} & \blue{471.45} & \blue{10.72} & / & \blue{482.17} \\ % 0.6014401912689209
& EgoNN \cite{komorowski2021egonn} & 109.87 & 0.14 & 21.75 & 131.76 \\
& \textbf{RING\#-L (Ours)} & 16.31 & 330.01 & / & 346.32 \\
% ICP Refinement 94.60
\bottomrule[1pt]
\end{tabular}
\begin{tablenotes}
    \footnotesize
    \item[$\dagger$] SS represents `SuperPoint + SuperGlue' for pose estimation after place recognition. We report the average runtime of each approach on ``2012-01-08'' to ``2012-08-20'' (the number of map keyframes in the database is 289) of the NCLT dataset.
\end{tablenotes}
\end{threeparttable}
\vspace{-0.2cm}
\end{table*}
